ALMACAL IX: multi-band ALMA survey for dusty star-forming galaxies and the resolved fractions of the cosmic infrared background

Wide, deep, blind continuum surveys at submillimetre/millimetre (submm/mm) wavelengths are required to provide a full inventory of the dusty, distant Universe. However, conducting such surveys to the necessary depth, with sub-arcsec angular resolution, is prohibitively time-consuming, even for the most advanced submm/mm telescopes. Here, we report the most recent results from the ALMACAL project, which exploits the 'free' calibration data from the Atacama Large Millimetre/submillimetre Array (ALMA) to map the lines of sight towards and beyond the ALMA calibrators. ALMACAL has now covered 1,001 calibrators, with a total sky coverage around 0.3 deg2, distributed across the sky accessible from the Atacama desert, and has accumulated more than 1,000h of integration. The depth reached by combining multiple visits to each field makes ALMACAL capable of searching for faint, dusty, star-forming galaxies (DSFGs), with detections at multiple frequencies to constrain the emission mechanism. Based on the most up-to-date ALMACAL database, we report the detection of 186 DSFGs with flux densities down to S870um ~ 0.2mJy, comparable with existing ALMA large surveys but less susceptible to cosmic variance. We report the number counts at five wavelengths between 870um and 3mm, in ALMA bands 3, 4, 5, 6 and 7, providing a benchmark for models of galaxy formation and evolution. By integrating the observed number counts and the best-fitting functions, we also present the resolved fraction of the cosmic infrared background (CIB) and the CIB spectral shape. Combining existing surveys, ALMA has currently resolved about half of the CIB in the submm/mm regime.

==> data/B3_catalogue_page0.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 3 }
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0026-3512 & 0 & 0 & 6.55748 & -35.21628 & 0.25 & 2.2 & 0.23 & 2.6 & 0.11 & 5.0 & 33.25\\
J0050-0929 & 0 & 2 & 12.67193 & -9.48647 & 1.56 & 24.4 & 2.17 & 20.7 & 0.80 & 23.3 & 6.12\\
J0112-6634 & 0 & 2 & 18.07620 & -66.57900 & 0.68 & 11.4 & 0.68 & 12.4 & 0.57 & 18.9 & 3.81\\
J0115-0127 & 0 & 2 & 18.82275 & -1.45256 & 1.41 & 24.7 & 1.78 & 19.1 & 0.76 & 22.3 & 7.11\\
J0137-2430 & 0 & 2 & 24.41549 & -24.51633 & 1.38 & 15.8 & 1.84 & 12.1 & 0.68 & 17.0 & 19.35\\
J0137-2430 & 1 & 2 & 24.40509 & -24.51524 & 2.19 & 26.1 & 2.52 & 21.9 & 1.26 & 31.8 & 15.38\\
J0141-0928 & 0 & 2 & 25.35748 & -9.47994 & 0.36 & 10.9 & 0.43 & 8.4 & 0.20 & 10.5 & 4.15\\
J0141-0928 & 1 & 2 & 25.35510 & -9.47481 & 0.17 & 4.0 & 0.16 & 3.1 & 0.10 & 5.2 & 16.95\\
J0220+3241 & 0 & 2 & 35.19971 & 32.68580 & 1.98 & 16.4 & 1.98 & 17.9 & 1.83 & 29.0 & 2.88\\
J0301+0118 & 0 & 2 & 45.34475 & 1.30914 & 0.15 & 2.9 & 0.15 & 4.0 & 0.13 & 10.5 & 13.37\\
J0301+0118 & 1 & 1 & 45.34219 & 1.31596 & 0.20 & 3.5 & 0.19 & 2.0 & 0.10 & 7.8 & 30.90\\
J0336+3218 & 0 & 2 & 54.12667 & 32.30643 & 1.17 & 20.9 & 1.40 & 17.3 & 0.69 & 19.3 & 7.24\\
J0411-5149 & 0 & 0 & 62.90926 & -51.82717 & 0.62 & 14.2 & 0.61 & 13.9 & 0.45 & 17.1 & 17.56\\
J0435+2532 & 0 & 2 & 68.89470 & 25.54751 & 0.23 & 7.8 & 0.37 & 5.6 & 0.07 & 5.0 & 8.89\\
J0438-1251 & 0 & 2 & 69.64725 & -12.85125 & 0.17 & 7.7 & 0.22 & 7.7 & 0.11 & 8.8 & 4.81\\
J0534-6106 & 0 & 0 & 83.65180 & -61.10192 & 0.32 & 4.8 & 0.35 & 4.6 & 0.30 & 6.3 & 4.79\\
J0541-0211 & 0 & 0 & 85.32777 & -2.18658 & 0.95 & 6.1 & 0.93 & 5.2 & 0.16 & 10.9 & 45.56\\
J0547+1223 & 0 & 0 & 86.78102 & 12.40447 & 0.44 & 3.0 & 0.48 & 3.1 & 0.19 & 5.2 & 34.41\\
J0559-4529 & 0 & 0 & 89.79820 & -45.49066 & 2.23 & 33.0 & 2.26 & 29.5 & 1.80 & 36.2 & 13.92\\
J0604+2429 & 0 & 2 & 91.23358 & 24.49893 & 1.17 & 23.6 & 1.34 & 20.2 & 0.74 & 26.2 & 12.84\\
J0613+1708 & 0 & 1 & 93.39150 & 17.13744 & 0.83 & 4.0 & 0.86 & 4.6 & 0.34 & 5.4 & 35.86\\
J0641-0320 & 0 & 2 & 100.46264 & -3.34814 & 0.73 & 5.1 & 0.74 & 5.8 & 0.73 & 10.1 & 4.96\\
J0808+0514 & 0 & 1 & 122.16652 & 5.24056 & 0.17 & 3.8 & 0.17 & 3.2 & 0.10 & 5.1 & 21.73\\
J0853+0654 & 0 & 2 & 133.45282 & 6.91731 & 7.10 & 100.7 & 13.38 & 71.4 & 1.75 & 63.1 & 16.74\\
J0909+0121 & 0 & 2 & 137.29556 & 1.35955 & 0.99 & 58.0 & 1.02 & 63.2 & 0.77 & 92.2 & 12.68\\
J0927-2034 & 0 & 2 & 141.96794 & -20.58623 & 2.42 & 23.2 & 5.09 & 15.3 & 0.93 & 21.6 & 20.36\\
J0927-2034 & 1 & 2 & 141.96706 & -20.57325 & 3.04 & 21.4 & 3.72 & 19.9 & 1.14 & 26.4 & 27.79\\
J0943-0819 & 0 & 2 & 145.91123 & -8.32244 & 0.48 & 4.6 & 0.51 & 5.3 & 0.30 & 7.8 & 27.83\\
J0946+1017 & 0 & 2 & 146.64780 & 10.28509 & 0.68 & 9.1 & 0.75 & 7.6 & 0.54 & 9.1 & 5.94\\
J0948+0022 & 0 & 2 & 147.23959 & 0.37616 & 0.12 & 18.0 & 0.12 & 16.2 & 0.10 & 30.0 & 9.03\\
J1000+0005 & 0 & 2 & 150.08182 & 0.09249 & 0.23 & 10.7 & 0.23 & 10.4 & 0.10 & 18.5 & 30.89\\
J1016+0513 & 0 & 1 & 154.01380 & 5.21554 & 0.08 & 3.3 & 0.09 & 3.1 & 0.07 & 5.6 & 6.90\\
J1036-3744 & 0 & 2 & 159.22084 & -37.72425 & 2.68 & 18.3 & 2.74 & 15.4 & 0.36 & 21.7 & 48.06\\
J1045+1735 & 0 & 2 & 161.31166 & 17.59463 & 0.39 & 3.6 & 0.38 & 3.0 & 0.47 & 5.8 & 9.71\\
J1107-4449 & 0 & 2 & 166.78355 & -44.81977 & 0.20 & 10.4 & 0.26 & 6.5 & 0.11 & 9.4 & 7.71\\
J1107-4449 & 1 & 2 & 166.79056 & -44.81399 & 0.38 & 8.0 & 0.40 & 7.7 & 0.22 & 18.0 & 20.48\\
J1107-4449 & 2 & 2 & 166.78800 & -44.81166 & 0.21 & 5.0 & 0.21 & 6.1 & 0.13 & 11.2 & 26.03\\
J1107-6820 & 0 & 0 & 166.80030 & -68.34839 & 0.86 & 20.0 & 0.96 & 16.8 & 0.65 & 20.7 & 4.89\\
J1148+1840 & 0 & 2 & 177.15831 & 18.66848 & 0.47 & 13.3 & 0.49 & 12.7 & 0.37 & 20.6 & 3.95\\
J1220+0203 & 0 & 2 & 185.05231 & 2.06261 & 0.74 & 15.0 & 0.98 & 18.6 & 0.37 & 19.5 & 10.54\\
J1220+0203 & 1 & 2 & 185.05476 & 2.06326 & 0.94 & 23.2 & 1.15 & 18.9 & 0.37 & 19.1 & 19.66\\
J1243+1622 & 0 & 2 & 190.99025 & 16.37980 & 10.78 & 59.5 & 11.02 & 61.9 & 9.24 & 92.4 & 6.13\\
J1243+1622 & 1 & 2 & 190.98911 & 16.38386 & 27.85 & 181.0 & 28.51 & 59.5 & 23.47 & 234.9 & 9.32\\
J1248-0632 & 0 & 1 & 192.09284 & -6.54367 & 0.28 & 2.9 & 0.25 & 2.7 & 0.14 & 5.3 & 29.28\\
J1315-5334 & 0 & 2 & 198.76949 & -53.57684 & 0.33 & 10.2 & 0.34 & 8.8 & 0.27 & 18.0 & 4.49\\

\hline
\end{tabular}
\flushleft
\emph{Note}: {The index represents the index of sources found in the same field. The types are SMG=1, Synchrotron=2, unclassified=0. The radial distance is the distance to the field centre.
\end{table}
\end{landscape}


==> data/B3_catalogue_page1.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 3 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J1315-5334 & 1 & 2 & 198.76350 & -53.57615 & 0.22 & 6.1 & 0.26 & 5.5 & 0.09 & 6.3 & 8.55\\
J1322-6532 & 0 & 2 & 200.72798 & -65.54200 & 0.53 & 6.9 & 0.67 & 4.8 & 0.20 & 5.9 & 12.40\\
J1333-2356 & 0 & 2 & 203.41246 & -23.93986 & 1.26 & 13.9 & 1.39 & 11.6 & 0.67 & 16.5 & 2.26\\
J1342-2900 & 0 & 0 & 205.57226 & -29.01743 & 0.58 & 17.3 & 0.65 & 16.3 & 0.17 & 17.9 & 33.49\\
J1342-3240 & 0 & 0 & 205.51230 & -32.68124 & 1.56 & 5.0 & 1.89 & 4.3 & 0.25 & 5.1 & 41.33\\
J1351-2912 & 0 & 0 & 207.94988 & -29.21147 & 0.14 & 3.3 & 0.12 & 2.9 & 0.08 & 5.4 & 27.92\\
J1353+1435 & 0 & 2 & 208.34418 & 14.59391 & 0.80 & 9.4 & 1.05 & 6.2 & 0.35 & 7.0 & 3.64\\
J1359+0159 & 0 & 2 & 209.85741 & 2.00221 & 0.17 & 5.6 & 0.18 & 5.0 & 0.10 & 6.8 & 24.53\\
J1408-2900 & 0 & 2 & 212.20532 & -29.00604 & 4.20 & 34.7 & 4.44 & 31.0 & 3.17 & 35.7 & 4.80\\
J1514+0252 & 0 & 2 & 228.64417 & 2.88300 & 0.21 & 6.6 & 0.27 & 5.5 & 0.11 & 5.3 & 10.49\\
J1832-1035 & 0 & 1 & 278.08118 & -10.57886 & 0.37 & 5.4 & 0.37 & 4.4 & 0.13 & 8.4 & 33.82\\
J1832-1035 & 1 & 1 & 278.08342 & -10.57696 & 0.40 & 2.5 & 0.41 & 3.2 & 0.09 & 5.0 & 36.18\\
J1907+0127 & 0 & 2 & 286.79770 & 1.45269 & 0.32 & 3.9 & 0.35 & 2.8 & 0.21 & 5.4 & 8.24\\
J2019-5201 & 0 & 0 & 304.76449 & -52.03010 & 0.23 & 5.3 & 0.27 & 4.8 & 0.15 & 5.9 & 12.27\\
J2049-4020 & 0 & 0 & 312.27783 & -40.34931 & 0.43 & 2.6 & 0.39 & 2.7 & 0.13 & 5.2 & 46.37\\
J2151-3027 & 0 & 2 & 327.98175 & -30.46573 & 1.69 & 14.2 & 1.71 & 13.4 & 1.40 & 19.9 & 3.18\\
J2207-5346 & 0 & 2 & 331.93405 & -53.77484 & 0.45 & 5.4 & 0.47 & 4.9 & 0.33 & 6.4 & 5.88\\
J2226+0052 & 0 & 1 & 336.69644 & 0.87313 & 0.07 & 3.8 & 0.07 & 3.7 & 0.06 & 6.1 & 15.03\\
J2335-0131 & 0 & 2 & 353.83611 & -1.51992 & 1.63 & 45.8 & 1.62 & 43.3 & 1.54 & 70.8 & 4.36\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B4_catalogue_page0.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 4 }
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0034-0054 & 0 & 1 & 8.68504 & -0.89826 & 0.46 & 4.1 & 0.43 & 3.1 & 0.21 & 6.1 & 20.62\\
J0034-0054 & 1 & 1 & 8.68317 & -0.89750 & 0.53 & 3.8 & 0.49 & 3.1 & 0.20 & 5.6 & 22.04\\
J0040-0146 & 0 & 2 & 10.23980 & -1.77435 & 0.27 & 3.7 & 0.26 & 3.7 & 0.22 & 5.4 & 4.46\\
J0132-1654 & 0 & 2 & 23.18106 & -16.91501 & 1.06 & 15.2 & 1.07 & 13.7 & 0.83 & 19.2 & 5.52\\
J0139+1753 & 0 & 1 & 24.92851 & 17.88339 & 0.37 & 6.6 & 0.36 & 6.3 & 0.26 & 11.1 & 14.34\\
J0139+1753 & 1 & 0 & 24.92091 & 17.88877 & 0.20 & 2.8 & 0.19 & 3.1 & 0.12 & 5.0 & 18.24\\
J0217-0820 & 0 & 1 & 34.26137 & -8.35057 & 0.20 & 4.2 & 0.20 & 4.6 & 0.21 & 7.0 & 9.74\\
J0217-0820 & 1 & 1 & 34.26296 & -8.34891 & 0.17 & 2.9 & 0.16 & 3.5 & 0.19 & 6.3 & 7.62\\
J0217-0820 & 2 & 2 & 34.26136 & -8.34703 & 0.98 & 19.6 & 0.98 & 18.7 & 0.77 & 25.9 & 3.17\\
J0217-0820 & 3 & 1 & 34.26225 & -8.34411 & 0.30 & 3.5 & 0.32 & 3.0 & 0.16 & 5.3 & 14.17\\
J0220+3241 & 0 & 2 & 35.19971 & 32.68580 & 1.29 & 15.5 & 1.28 & 14.1 & 1.15 & 29.4 & 2.87\\
J0224+0659 & 0 & 2 & 36.11433 & 6.99064 & 1.32 & 6.9 & 1.99 & 5.9 & 0.34 & 5.8 & 15.06\\
J0243-0550 & 0 & 1 & 40.80245 & -5.85391 & 0.30 & 7.3 & 0.32 & 7.9 & 0.15 & 10.9 & 18.87\\
J0336-1302 & 0 & 2 & 54.14650 & -13.03332 & 0.37 & 8.3 & 0.38 & 8.0 & 0.32 & 10.2 & 5.06\\
J0348-2749 & 0 & 1 & 57.15576 & -27.82009 & 0.11 & 4.6 & 0.14 & 2.2 & 0.06 & 5.1 & 10.20\\
J0407-1211 & 0 & 2 & 61.95061 & -12.19706 & 2.21 & 30.4 & 2.47 & 33.6 & 0.77 & 38.7 & 13.40\\
J0428-6438 & 0 & 1 & 67.06182 & -64.63583 & 1.15 & 6.3 & 1.28 & 3.8 & 0.18 & 6.0 & 29.21\\
J0526-6749 & 0 & 1 & 81.66800 & -67.82271 & 1.20 & 3.8 & 1.17 & 3.1 & 0.20 & 5.3 & 31.45\\
J0527-1002 & 0 & 0 & 81.84343 & -10.05150 & 0.61 & 2.9 & 0.58 & 2.9 & 0.19 & 5.9 & 25.52\\
J0527-1002 & 1 & 0 & 81.84766 & -10.04838 & 0.18 & 2.4 & 0.17 & 2.6 & 0.19 & 5.7 & 9.70\\
J0748+2400 & 0 & 2 & 117.15210 & 24.00734 & 1.05 & 5.7 & 1.38 & 4.1 & 0.41 & 5.0 & 5.89\\
J0839+0104 & 0 & 2 & 129.95509 & 1.07344 & 0.48 & 7.3 & 0.53 & 6.8 & 0.33 & 8.5 & 6.31\\
J0853+0654 & 0 & 2 & 133.45281 & 6.91734 & 7.27 & 26.9 & 9.67 & 20.2 & 2.33 & 21.4 & 16.83\\
J0909+0121 & 0 & 2 & 137.29558 & 1.35952 & 0.68 & 8.6 & 0.74 & 9.0 & 0.45 & 12.0 & 12.78\\
J0927-2034 & 0 & 2 & 141.96798 & -20.58623 & 1.76 & 21.1 & 3.85 & 16.4 & 0.41 & 15.6 & 20.40\\
J0927-2034 & 1 & 2 & 141.96706 & -20.57326 & 2.30 & 13.4 & 2.80 & 12.2 & 0.38 & 14.6 & 27.75\\
J0948+0022 & 0 & 1 & 147.24147 & 0.36969 & 0.11 & 6.7 & 0.11 & 5.1 & 0.06 & 9.6 & 17.46\\
J0948+0022 & 1 & 2 & 147.23960 & 0.37620 & 0.08 & 6.9 & 0.09 & 6.7 & 0.07 & 10.2 & 9.19\\
J1008+0621 & 0 & 1 & 152.00431 & 6.36130 & 0.21 & 4.6 & 0.22 & 3.6 & 0.09 & 6.3 & 19.75\\
J1130-1449 & 0 & 1 & 172.53411 & -14.82108 & 0.19 & 3.0 & 0.19 & 2.7 & 0.10 & 5.2 & 20.05\\
J1146-2447 & 0 & 1 & 176.53057 & -24.78945 & 0.26 & 5.9 & 0.25 & 6.2 & 0.17 & 8.3 & 15.07\\
J1220+0203 & 0 & 2 & 185.05235 & 2.06257 & 0.60 & 6.9 & 0.61 & 9.0 & 0.38 & 9.7 & 10.62\\
J1220+0203 & 1 & 2 & 185.05472 & 2.06322 & 0.90 & 6.2 & 0.99 & 7.0 & 0.34 & 8.7 & 19.47\\
J1254+1141 & 0 & 2 & 193.65766 & 11.68606 & 0.38 & 8.2 & 0.60 & 6.3 & 0.19 & 7.0 & 7.28\\
J1332-0509 & 0 & 0 & 203.01910 & -5.15930 & 0.47 & 9.7 & 0.59 & 7.8 & 0.18 & 8.4 & 9.97\\
J1353+1435 & 0 & 0 & 208.34421 & 14.59399 & 0.64 & 6.9 & 0.88 & 4.7 & 0.29 & 5.4 & 3.45\\
J1419+2706 & 0 & 0 & 214.99622 & 27.11259 & 0.33 & 3.4 & 0.32 & 3.5 & 0.19 & 5.0 & 19.96\\
J1454-3747 & 0 & 2 & 223.62288 & -37.79092 & 1.06 & 6.5 & 2.01 & 4.3 & 0.12 & 5.2 & 25.34\\
J1454-3747 & 1 & 1 & 223.61394 & -37.79078 & 0.43 & 8.0 & 0.41 & 8.7 & 0.38 & 16.0 & 6.37\\
J1534+0131 & 0 & 0 & 233.71691 & 1.51622 & 0.38 & 3.6 & 0.37 & 2.9 & 0.23 & 5.3 & 8.31\\
J1540+1447 & 0 & 0 & 235.21325 & 14.79725 & 0.79 & 5.7 & 0.79 & 5.3 & 0.22 & 5.4 & 24.86\\
J1550+0527 & 0 & 1 & 237.64211 & 5.45486 & 0.10 & 1.5 & 0.10 & 3.9 & 0.06 & 7.1 & 18.74\\
J1555+1111 & 0 & 1 & 238.93224 & 11.18728 & 0.17 & 4.9 & 0.16 & 5.4 & 0.13 & 7.9 & 14.39\\
J1555+1111 & 1 & 1 & 238.92983 & 11.19516 & 0.16 & 3.5 & 0.16 & 3.1 & 0.09 & 5.4 & 18.30\\
J1733-1304 & 0 & 2 & 263.25812 & -13.08024 & 3.22 & 12.8 & 3.43 & 12.3 & 2.13 & 15.5 & 11.08\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B4_catalogue_page1.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 4 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J1733-3722 & 0 & 1 & 263.31336 & -37.37359 & 0.44 & 7.6 & 0.48 & 5.8 & 0.26 & 9.7 & 7.46\\
J1751-1950 & 0 & 2 & 267.92227 & -19.84774 & 0.11 & 2.9 & 0.11 & 3.1 & 0.12 & 6.7 & 4.38\\
J1851+0035 & 0 & 1 & 282.94912 & 0.59527 & 0.36 & 1.7 & 0.36 & 2.5 & 0.21 & 8.2 & 19.19\\
J1924-2914 & 0 & 2 & 291.21240 & -29.24233 & 0.78 & 6.9 & 1.15 & 6.7 & 0.26 & 5.8 & 2.51\\
J2025-0735 & 0 & 2 & 306.41913 & -7.59742 & 6.55 & 37.8 & 6.68 & 33.1 & 5.12 & 58.0 & 2.24\\
J2141-6411 & 0 & 0 & 325.42887 & -64.18656 & 0.82 & 3.0 & 0.76 & 3.5 & 0.30 & 5.3 & 23.12\\
J2316+1618 & 0 & 0 & 349.16685 & 16.29818 & 0.28 & 4.8 & 0.31 & 4.1 & 0.09 & 5.0 & 14.21\\
J2316+1618 & 1 & 0 & 349.16622 & 16.30226 & 0.42 & 11.0 & 0.47 & 9.5 & 0.21 & 11.3 & 3.12\\
J2357-5311 & 0 & 1 & 359.46859 & -53.19167 & 0.08 & 3.6 & 0.08 & 2.3 & 0.04 & 5.4 & 17.84\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B5_catalogue_page0.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 5 }
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0108+0135 & 0 & 2 & 17.16147 & 1.58222 & 1.92 & 9.1 & 2.05 & 7.1 & 1.28 & 11.5 & 4.33\\
J0108+0135 & 1 & 0 & 17.16278 & 1.58838 & 1.65 & 3.4 & 1.89 & 3.0 & 0.56 & 5.1 & 18.38\\
J0217-0820 & 0 & 1 & 34.26137 & -8.35057 & 0.42 & 2.1 & 0.48 & 3.9 & 0.52 & 6.4 & 9.77\\
J0217-0820 & 1 & 1 & 34.26298 & -8.34884 & 0.58 & 3.6 & 0.58 & 3.9 & 0.58 & 7.2 & 7.56\\
J0217-0820 & 2 & 2 & 34.26144 & -8.34709 & 0.79 & 7.9 & 0.81 & 5.1 & 0.53 & 6.6 & 3.08\\
J0407-1211 & 0 & 2 & 61.95063 & -12.19710 & 2.05 & 6.2 & 2.27 & 5.0 & 0.73 & 7.2 & 13.53\\
J0407-1211 & 1 & 2 & 61.95247 & -12.18838 & 9.12 & 17.6 & 9.26 & 17.1 & 2.83 & 28.1 & 18.64\\
J0948+0022 & 0 & 1 & 147.24150 & 0.36969 & 0.42 & 6.0 & 0.43 & 4.4 & 0.12 & 6.2 & 17.54\\
J1058+0133 & 0 & 1 & 164.62386 & 1.56589 & 1.09 & 12.2 & 1.20 & 10.4 & 0.79 & 19.1 & 2.43\\
J1107-4449 & 0 & 1 & 166.78498 & -44.82355 & 0.51 & 4.9 & 0.54 & 4.4 & 0.18 & 7.8 & 17.47\\
J1550+0527 & 0 & 1 & 237.64219 & 5.45487 & 0.37 & 3.8 & 0.38 & 4.0 & 0.11 & 6.6 & 18.49\\
J1625-2527 & 0 & 1 & 246.44291 & -25.46531 & 0.62 & 2.3 & 0.58 & 2.3 & 0.26 & 5.7 & 18.61\\
J1730+0024 & 0 & 0 & 262.64690 & 0.41069 & 0.11 & 1.5 & 0.12 & 2.3 & 0.18 & 5.4 & 3.85\\
J1733-1304 & 0 & 2 & 263.25816 & -13.08024 & 1.68 & 7.6 & 1.86 & 7.1 & 0.71 & 8.7 & 10.95\\
J1733-3722 & 0 & 1 & 263.31342 & -37.37362 & 0.94 & 7.6 & 0.92 & 6.0 & 0.64 & 9.5 & 7.37\\
J1851+0035 & 0 & 2 & 282.94407 & 0.59134 & 0.98 & 13.6 & 1.00 & 17.3 & 0.81 & 21.4 & 4.17\\
J1851+0035 & 1 & 1 & 282.94921 & 0.59530 & 1.62 & 8.4 & 1.67 & 4.0 & 0.34 & 9.0 & 19.51\\
J2056-4714 & 0 & 2 & 314.06715 & -47.24762 & 0.31 & 7.9 & 0.34 & 7.5 & 0.18 & 10.2 & 4.53\\
J2207-5346 & 0 & 2 & 331.93111 & -53.77732 & 1.28 & 17.6 & 1.54 & 15.0 & 0.74 & 21.9 & 5.11\\
J2258-2758 & 0 & 1 & 344.52212 & -27.97566 & 0.48 & 4.0 & 0.55 & 3.0 & 0.16 & 5.4 & 14.09\\
J2258-2758 & 1 & 2 & 344.52262 & -27.97194 & 0.24 & 3.2 & 0.25 & 2.7 & 0.16 & 5.2 & 7.44\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B6_catalogue_page0.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 6 }
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0004-1148 & 0 & 1 & 1.01928 & -11.81916 & 1.00 & 7.5 & 1.06 & 6.3 & 0.39 & 10.5 & 11.40\\
J0019+2021 & 0 & 1 & 4.90608 & 20.36282 & 0.57 & 8.4 & 0.64 & 8.4 & 0.37 & 10.7 & 5.60\\
J0045-3705 & 0 & 1 & 11.29664 & -37.09474 & 0.17 & 2.6 & 0.16 & 2.8 & 0.10 & 5.9 & 12.80\\
J0049-4457 & 0 & 1 & 12.32260 & -44.94920 & 1.44 & 4.5 & 1.34 & 4.1 & 0.33 & 7.1 & 16.43\\
J0050-0452 & 0 & 1 & 12.58663 & -4.87507 & 1.61 & 11.0 & 1.58 & 10.3 & 0.49 & 16.5 & 14.74\\
J0106-2718 & 0 & 1 & 16.61071 & -27.30215 & 1.08 & 14.4 & 1.10 & 13.8 & 0.66 & 23.1 & 7.68\\
J0108+0135 & 0 & 1 & 17.16107 & 1.57858 & 1.12 & 2.7 & 1.22 & 3.0 & 0.17 & 6.0 & 17.53\\
J0108+0135 & 1 & 2 & 17.16145 & 1.58221 & 0.92 & 15.6 & 0.92 & 17.5 & 0.81 & 28.0 & 4.37\\
J0108+0135 & 2 & 1 & 17.16065 & 1.58451 & 1.10 & 19.1 & 1.10 & 20.3 & 0.90 & 31.3 & 5.07\\
J0113-3551 & 0 & 1 & 18.31699 & -35.86773 & 0.84 & 4.4 & 0.85 & 4.6 & 0.20 & 7.4 & 15.69\\
J0120-2701 & 0 & 1 & 20.13225 & -27.02218 & 0.88 & 11.3 & 0.98 & 7.9 & 0.52 & 14.5 & 4.92\\
J0125-0005 & 0 & 1 & 21.36913 & -0.09499 & 1.09 & 5.0 & 1.22 & 3.9 & 0.21 & 5.2 & 14.49\\
J0126-2222 & 0 & 2 & 21.56312 & -22.37618 & 2.99 & 26.3 & 3.15 & 19.2 & 2.39 & 26.4 & 2.16\\
J0132-1654 & 0 & 2 & 23.18111 & -16.91501 & 0.64 & 6.8 & 0.73 & 5.1 & 0.42 & 7.7 & 5.51\\
J0139+1753 & 0 & 1 & 24.92850 & 17.88337 & 1.48 & 11.5 & 1.49 & 13.7 & 0.53 & 20.0 & 14.33\\
J0153-3310 & 0 & 0 & 28.28999 & -33.17349 & 0.53 & 5.3 & 0.53 & 5.4 & 0.51 & 7.6 & 6.70\\
J0154+0823 & 0 & 0 & 28.51240 & 8.39700 & 0.76 & 3.5 & 0.80 & 3.3 & 0.41 & 5.5 & 3.57\\
J0215-0222 & 0 & 2 & 33.92506 & -2.38317 & 0.33 & 6.7 & 0.34 & 5.0 & 0.27 & 9.4 & 2.67\\
J0217-0820 & 0 & 1 & 34.26137 & -8.35057 & 1.44 & 26.4 & 1.45 & 42.7 & 0.76 & 90.4 & 9.75\\
J0217-0820 & 1 & 1 & 34.26030 & -8.34989 & 0.13 & 6.4 & 0.15 & 2.6 & 0.07 & 8.9 & 7.77\\
J0217-0820 & 2 & 1 & 34.26220 & -8.34892 & 0.11 & 3.4 & 0.11 & 3.8 & 0.09 & 11.0 & 5.45\\
J0217-0820 & 3 & 1 & 34.26291 & -8.34891 & 1.43 & 29.0 & 1.52 & 12.5 & 0.76 & 90.3 & 7.48\\
J0217-0820 & 4 & 2 & 34.26137 & -8.34700 & 0.53 & 6.4 & 0.53 & 17.4 & 0.40 & 47.3 & 3.29\\
J0217-0820 & 5 & 1 & 34.25876 & -8.34578 & 0.13 & 1.3 & 0.13 & 3.9 & 0.06 & 6.9 & 11.23\\
J0217-0820 & 6 & 1 & 34.26226 & -8.34416 & 1.23 & 18.4 & 1.26 & 6.7 & 0.40 & 47.9 & 14.01\\
J0220+3241 & 0 & 1 & 35.20415 & 32.68315 & 1.65 & 6.1 & 1.82 & 5.8 & 0.48 & 8.0 & 13.87\\
J0220+3241 & 1 & 2 & 35.19971 & 32.68579 & 0.77 & 6.3 & 0.74 & 6.4 & 0.68 & 11.4 & 2.83\\
J0228-0337 & 0 & 1 & 37.22007 & -3.62701 & 0.36 & 8.1 & 0.36 & 6.7 & 0.27 & 11.2 & 5.89\\
J0228-0337 & 1 & 1 & 37.22639 & -3.62569 & 0.84 & 4.9 & 0.91 & 4.2 & 0.16 & 6.5 & 17.41\\
J0238+1636 & 0 & 1 & 39.66496 & 16.61566 & 0.24 & 5.2 & 0.24 & 4.8 & 0.10 & 8.6 & 9.91\\
J0239+0416 & 0 & 2 & 39.96314 & 4.27328 & 0.31 & 3.5 & 0.30 & 3.2 & 0.27 & 7.0 & 2.91\\
J0239-0234 & 0 & 1 & 39.93741 & -2.57802 & 0.24 & 6.0 & 0.26 & 6.6 & 0.09 & 8.6 & 7.41\\
J0239-0234 & 1 & 1 & 39.93726 & -2.57456 & 0.63 & 7.4 & 0.64 & 8.6 & 0.18 & 16.5 & 14.83\\
J0241-0815 & 0 & 2 & 40.27096 & -8.25540 & 0.19 & 4.7 & 0.33 & 3.7 & 0.08 & 5.0 & 3.69\\
J0241-0815 & 1 & 1 & 40.27006 & -8.25416 & 0.55 & 13.9 & 0.54 & 13.6 & 0.42 & 26.7 & 5.79\\
J0243-0550 & 0 & 1 & 40.80249 & -5.85388 & 3.24 & 12.5 & 3.19 & 10.6 & 0.44 & 17.6 & 18.75\\
J0253-5441 & 0 & 0 & 43.37278 & -54.69965 & 0.90 & 11.6 & 0.93 & 7.2 & 0.55 & 18.7 & 7.72\\
J0253-5441 & 1 & 1 & 43.37232 & -54.69618 & 0.47 & 9.5 & 0.47 & 6.7 & 0.33 & 11.4 & 5.40\\
J0301+0118 & 0 & 2 & 45.34761 & 1.31034 & 0.68 & 4.0 & 0.79 & 3.1 & 0.39 & 5.8 & 2.98\\
J0329-2357 & 0 & 2 & 52.47285 & -23.95234 & 0.21 & 4.7 & 0.25 & 4.1 & 0.09 & 5.8 & 8.14\\
J0336-1302 & 0 & 1 & 54.14794 & -13.03755 & 0.61 & 5.8 & 0.62 & 4.7 & 0.21 & 5.7 & 12.55\\
J0339-0146 & 0 & 2 & 54.87855 & -1.77524 & 0.57 & 7.2 & 0.60 & 6.5 & 0.45 & 10.6 & 5.12\\
J0348-2749 & 0 & 2 & 57.15949 & -27.82073 & 1.26 & 55.9 & 1.27 & 55.1 & 0.99 & 127.8 & 2.04\\
J0348-2749 & 1 & 1 & 57.15578 & -27.82014 & 0.35 & 9.9 & 0.40 & 9.0 & 0.12 & 15.2 & 10.11\\
J0407-1211 & 0 & 2 & 61.95061 & -12.19704 & 1.64 & 7.5 & 1.93 & 6.7 & 0.41 & 8.1 & 13.35\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B6_catalogue_page1.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 6 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0407-1211 & 1 & 2 & 61.95247 & -12.18838 & 5.76 & 11.2 & 5.88 & 10.1 & 0.96 & 18.9 & 18.65\\
J0423-0120 & 0 & 1 & 65.81293 & -1.34117 & 0.18 & 3.6 & 0.19 & 3.2 & 0.10 & 7.2 & 11.54\\
J0425-5331 & 0 & 2 & 66.26875 & -53.53264 & 0.38 & 10.7 & 0.40 & 8.1 & 0.29 & 11.2 & 2.16\\
J0426+2327 & 0 & 1 & 66.73750 & 23.46230 & 0.61 & 4.0 & 0.65 & 3.9 & 0.07 & 5.2 & 18.00\\
J0426+2327 & 1 & 1 & 66.73112 & 23.46269 & 0.20 & 6.0 & 0.24 & 4.9 & 0.08 & 6.2 & 7.11\\
J0427+0457 & 0 & 2 & 66.94845 & 4.95312 & 1.04 & 14.0 & 1.28 & 12.3 & 0.49 & 13.8 & 3.02\\
J0433+0521 & 0 & 2 & 68.29518 & 5.35420 & 3.01 & 7.6 & 3.78 & 6.8 & 1.66 & 8.5 & 3.80\\
J0438+3004 & 0 & 1 & 69.52086 & 30.07534 & 0.58 & 3.3 & 0.61 & 6.0 & 0.13 & 10.9 & 14.28\\
J0439+3045 & 0 & 0 & 69.82537 & 30.75194 & 1.37 & 21.4 & 1.37 & 18.8 & 1.02 & 36.2 & 4.10\\
J0455-4615 & 0 & 0 & 73.96256 & -46.26782 & 1.28 & 5.8 & 1.39 & 3.7 & 0.70 & 7.7 & 6.02\\
J0455-4615 & 1 & 0 & 73.96007 & -46.26550 & 0.85 & 1.8 & 0.86 & 4.1 & 0.65 & 7.1 & 4.68\\
J0457-2324 & 0 & 1 & 74.26507 & -23.41668 & 0.46 & 3.2 & 0.44 & 3.1 & 0.28 & 6.5 & 10.02\\
J0501-0159 & 0 & 1 & 75.30354 & -1.98785 & 0.52 & 5.7 & 0.64 & 6.7 & 0.30 & 10.4 & 2.06\\
J0502+0609 & 0 & 0 & 75.56507 & 6.15241 & 0.53 & 6.0 & 0.58 & 6.0 & 0.32 & 6.9 & 2.79\\
J0502+0609 & 1 & 0 & 75.56486 & 6.15573 & 0.89 & 5.9 & 0.86 & 4.2 & 0.40 & 8.6 & 13.26\\
J0511-6806 & 0 & 1 & 77.87265 & -68.10729 & 0.43 & 4.2 & 0.59 & 3.6 & 0.23 & 5.0 & 8.89\\
J0512+2927 & 0 & 1 & 78.17249 & 29.44962 & 1.74 & 12.2 & 1.71 & 12.8 & 0.72 & 24.4 & 11.68\\
J0521+2112 & 0 & 1 & 80.43609 & 21.21370 & 1.04 & 4.2 & 0.97 & 3.5 & 0.17 & 7.3 & 18.36\\
J0536-3401 & 0 & 1 & 84.11595 & -34.01856 & 0.28 & 5.3 & 0.28 & 5.3 & 0.19 & 7.4 & 8.82\\
J0538-4405 & 0 & 2 & 84.70677 & -44.08726 & 0.61 & 8.4 & 0.78 & 4.3 & 0.24 & 8.2 & 9.48\\
J0538-4405 & 1 & 1 & 84.70450 & -44.08709 & 0.50 & 3.3 & 0.60 & 2.9 & 0.15 & 5.2 & 14.54\\
J0541-0541 & 0 & 2 & 85.40953 & -5.69639 & 0.36 & 11.7 & 0.40 & 12.1 & 0.21 & 14.1 & 3.86\\
J0542-0913 & 0 & 1 & 85.73255 & -9.22695 & 0.10 & 1.8 & 0.11 & 2.6 & 0.07 & 7.1 & 6.09\\
J0542-0913 & 1 & 1 & 85.72931 & -9.22412 & 1.22 & 24.8 & 1.23 & 25.9 & 0.54 & 51.0 & 13.17\\
J0550-5732 & 0 & 1 & 87.53636 & -57.53790 & 0.41 & 3.7 & 0.40 & 3.0 & 0.23 & 5.9 & 10.53\\
J0601-7036 & 0 & 1 & 90.28902 & -70.60540 & 0.25 & 4.6 & 0.32 & 3.4 & 0.04 & 5.0 & 14.17\\
J0601-7036 & 1 & 1 & 90.30679 & -70.60001 & 0.35 & 5.9 & 0.35 & 5.7 & 0.09 & 10.6 & 14.75\\
J0607-0834 & 0 & 2 & 92.00013 & -8.58075 & 0.25 & 4.2 & 0.31 & 3.6 & 0.10 & 6.0 & 4.94\\
J0641-0320 & 0 & 2 & 100.46263 & -3.34811 & 0.33 & 7.4 & 0.35 & 4.6 & 0.23 & 8.8 & 4.86\\
J0641-0320 & 1 & 1 & 100.45921 & -3.34771 & 0.68 & 6.8 & 0.68 & 4.9 & 0.25 & 9.6 & 14.16\\
J0641-0320 & 2 & 1 & 100.46313 & -3.34607 & 0.36 & 8.4 & 0.38 & 5.5 & 0.29 & 10.7 & 2.73\\
J0641-0320 & 3 & 1 & 100.46230 & -3.34452 & 0.49 & 7.5 & 0.50 & 7.0 & 0.34 & 12.6 & 8.74\\
J0648-3044 & 0 & 0 & 102.05671 & -30.73851 & 0.28 & 3.6 & 0.26 & 3.1 & 0.18 & 5.1 & 6.34\\
J0656-0323 & 0 & 0 & 104.04682 & -3.38635 & 0.44 & 3.7 & 0.50 & 3.2 & 0.21 & 5.2 & 4.42\\
J0702-1015 & 0 & 0 & 105.65041 & -10.25300 & 0.41 & 7.2 & 0.40 & 6.7 & 0.31 & 9.4 & 6.69\\
J0750+1231 & 0 & 1 & 117.71508 & 12.52179 & 0.34 & 4.2 & 0.35 & 5.0 & 0.09 & 7.8 & 15.02\\
J0815+3635 & 0 & 2 & 123.85862 & 36.58675 & 0.91 & 10.1 & 0.92 & 10.5 & 0.78 & 15.3 & 3.22\\
J0831+0429 & 0 & 1 & 127.95458 & 4.49516 & 1.45 & 9.1 & 1.50 & 9.5 & 1.09 & 14.8 & 4.81\\
J0839+0104 & 0 & 2 & 129.95519 & 1.07346 & 0.31 & 7.7 & 0.32 & 7.2 & 0.23 & 10.1 & 5.94\\
J0839+0104 & 1 & 1 & 129.95469 & 1.07733 & 0.34 & 3.7 & 0.33 & 3.7 & 0.15 & 6.7 & 13.77\\
J0849-3541 & 0 & 0 & 132.44229 & -35.68318 & 0.34 & 6.6 & 0.33 & 5.5 & 0.25 & 10.5 & 6.67\\
J0849-3541 & 1 & 0 & 132.44082 & -35.68295 & 1.84 & 37.9 & 2.12 & 32.4 & 0.85 & 35.3 & 3.39\\
J0849-3541 & 2 & 0 & 132.44070 & -35.68078 & 0.47 & 5.3 & 0.61 & 4.4 & 0.13 & 5.5 & 10.60\\
J0853+0654 & 0 & 1 & 133.45060 & 6.91178 & 1.20 & 13.3 & 1.22 & 12.3 & 1.00 & 20.6 & 4.86\\
J0853+0654 & 1 & 2 & 133.45283 & 6.91739 & 3.44 & 11.0 & 4.92 & 10.7 & 0.48 & 9.9 & 17.02\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B6_catalogue_page2.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 6 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0854+2006 & 0 & 1 & 133.70594 & 20.10955 & 0.62 & 5.8 & 0.67 & 4.4 & 0.27 & 9.3 & 8.60\\
J0904-5735 & 0 & 1 & 136.21762 & -57.58284 & 0.98 & 4.7 & 1.02 & 1.6 & 0.46 & 9.8 & 10.77\\
J0919-5340 & 0 & 0 & 139.92821 & -53.67107 & 5.38 & 5.5 & 5.92 & 5.1 & 1.14 & 8.0 & 14.68\\
J0919-5340 & 1 & 0 & 139.92850 & -53.67057 & 8.26 & 10.5 & 9.58 & 9.1 & 1.57 & 11.1 & 13.09\\
J0922-0529 & 0 & 0 & 140.60398 & -5.48599 & 0.94 & 4.3 & 0.90 & 3.7 & 0.10 & 5.9 & 19.30\\
J0930+0034 & 0 & 1 & 142.71578 & 0.58266 & 0.31 & 2.6 & 0.27 & 2.7 & 0.32 & 5.7 & 7.11\\
J0942-0759 & 0 & 1 & 145.58785 & -7.99551 & 0.37 & 4.4 & 0.36 & 4.4 & 0.23 & 8.2 & 10.91\\
J0948+0022 & 0 & 1 & 147.24148 & 0.36971 & 0.58 & 10.7 & 0.56 & 10.9 & 0.12 & 28.5 & 17.45\\
J0948+0022 & 1 & 1 & 147.24084 & 0.37498 & 0.10 & 6.8 & 0.11 & 7.1 & 0.05 & 12.6 & 8.42\\
J0948+0022 & 2 & 2 & 147.23963 & 0.37620 & 0.06 & 3.4 & 0.06 & 2.5 & 0.04 & 8.3 & 9.23\\
J0948+0022 & 3 & 1 & 147.24173 & 0.37631 & 0.09 & 3.8 & 0.10 & 1.6 & 0.03 & 6.0 & 13.86\\
J0948+0022 & 4 & 1 & 147.23890 & 0.37660 & 0.09 & 3.0 & 0.10 & 3.7 & 0.03 & 7.3 & 10.20\\
J1008+0621 & 0 & 1 & 152.00423 & 6.36122 & 0.85 & 4.0 & 0.89 & 4.3 & 0.12 & 7.8 & 19.43\\
J1010-0200 & 0 & 1 & 152.71258 & -2.00521 & 0.17 & 5.0 & 0.17 & 3.4 & 0.09 & 13.3 & 9.76\\
J1010-0200 & 1 & 1 & 152.71299 & -2.00267 & 0.26 & 3.9 & 0.27 & 6.1 & 0.09 & 13.1 & 12.96\\
J1014+2301 & 0 & 0 & 153.69639 & 23.01806 & 1.80 & 6.4 & 2.63 & 4.3 & 0.57 & 5.4 & 11.61\\
J1016+0513 & 0 & 1 & 154.01110 & 5.21221 & 2.23 & 2.4 & 1.80 & 2.4 & 0.42 & 5.1 & 19.70\\
J1047-6217 & 0 & 1 & 161.92951 & -62.28652 & 0.29 & 6.5 & 0.29 & 6.7 & 0.20 & 9.3 & 3.30\\
J1051-3138 & 0 & 0 & 162.76972 & -31.64114 & 0.36 & 3.0 & 0.36 & 2.7 & 0.11 & 5.1 & 13.82\\
J1058+0133 & 0 & 1 & 164.62388 & 1.56590 & 1.82 & 10.2 & 1.87 & 24.6 & 1.38 & 55.7 & 2.45\\
J1107-4449 & 0 & 1 & 166.78498 & -44.82354 & 1.05 & 8.8 & 1.04 & 5.5 & 0.18 & 18.8 & 17.41\\
J1107-4449 & 1 & 1 & 166.78989 & -44.82198 & 0.30 & 5.3 & 0.39 & 3.2 & 0.05 & 5.1 & 14.81\\
J1107-4449 & 2 & 1 & 166.78458 & -44.81682 & 0.11 & 3.3 & 0.10 & 2.7 & 0.09 & 9.3 & 8.23\\
J1107-4449 & 3 & 1 & 166.79303 & -44.81662 & 0.57 & 4.2 & 0.57 & 4.2 & 0.10 & 10.1 & 19.01\\
J1118+1234 & 0 & 2 & 169.73824 & 12.57874 & 1.79 & 40.7 & 1.83 & 27.2 & 1.41 & 56.9 & 2.54\\
J1118+1234 & 1 & 1 & 169.74092 & 12.57934 & 0.77 & 13.6 & 0.79 & 11.6 & 0.46 & 18.4 & 8.53\\
J1118-4634 & 0 & 0 & 169.60572 & -46.56888 & 1.74 & 3.5 & 1.61 & 3.3 & 0.37 & 5.2 & 17.80\\
J1121-0553 & 0 & 1 & 170.35425 & -5.89973 & 2.20 & 14.2 & 2.18 & 12.5 & 1.75 & 19.1 & 2.91\\
J1127-1857 & 0 & 1 & 171.77147 & -18.95321 & 0.40 & 2.6 & 0.37 & 2.7 & 0.16 & 5.2 & 12.28\\
J1130-1449 & 0 & 1 & 172.53405 & -14.82104 & 1.96 & 5.8 & 2.14 & 3.8 & 0.23 & 5.6 & 19.99\\
J1147-0724 & 0 & 1 & 176.96365 & -7.41032 & 0.50 & 10.0 & 0.49 & 10.6 & 0.39 & 13.8 & 5.74\\
J1148+1840 & 0 & 1 & 177.15967 & 18.67130 & 1.18 & 14.8 & 1.21 & 15.5 & 0.59 & 26.0 & 10.93\\
J1150+2417 & 0 & 1 & 177.57915 & 24.29909 & 0.33 & 5.3 & 0.30 & 3.7 & 0.25 & 6.2 & 4.12\\
J1206-6138 & 0 & 0 & 181.71108 & -61.64867 & 0.18 & 4.8 & 0.21 & 3.0 & 0.09 & 5.5 & 6.16\\
J1206-6138 & 1 & 0 & 181.70896 & -61.64712 & 1.69 & 31.6 & 1.69 & 27.5 & 0.82 & 50.2 & 11.95\\
J1208-7809 & 0 & 1 & 182.08036 & -78.16033 & 0.73 & 4.9 & 0.75 & 4.7 & 0.31 & 7.0 & 11.78\\
J1215+1654 & 0 & 0 & 183.76413 & 16.91086 & 0.27 & 6.1 & 0.34 & 8.2 & 0.11 & 8.8 & 8.51\\
J1220+0203 & 0 & 1 & 185.04667 & 2.06255 & 0.27 & 4.4 & 0.35 & 3.3 & 0.10 & 5.7 & 10.68\\
J1220+0203 & 1 & 2 & 185.05220 & 2.06264 & 0.32 & 5.0 & 0.38 & 3.4 & 0.11 & 6.2 & 10.17\\
J1224+0330 & 0 & 0 & 186.21831 & 3.51327 & 2.41 & 44.9 & 2.41 & 55.9 & 2.09 & 86.8 & 2.55\\
J1224+0330 & 1 & 1 & 186.21533 & 3.51450 & 0.35 & 6.4 & 0.38 & 2.7 & 0.16 & 6.1 & 11.28\\
J1229-6003 & 0 & 0 & 187.36103 & -60.05965 & 2.61 & 9.5 & 2.79 & 8.3 & 2.01 & 10.7 & 2.96\\
J1243+1622 & 0 & 2 & 190.99027 & 16.37980 & 2.93 & 16.5 & 3.29 & 6.1 & 1.49 & 16.8 & 6.12\\
J1243+1622 & 1 & 2 & 190.98911 & 16.38388 & 13.32 & 57.5 & 14.08 & 50.2 & 6.46 & 73.1 & 9.37\\
J1246-0730 & 0 & 1 & 191.52136 & -7.51324 & 0.71 & 5.4 & 0.73 & 5.2 & 0.30 & 9.8 & 13.36\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B6_catalogue_page3.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 6 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J1252-6737 & 0 & 1 & 193.18191 & -67.63067 & 0.56 & 2.7 & 0.56 & 3.1 & 0.39 & 6.6 & 11.94\\
J1254+1141 & 0 & 2 & 193.65773 & 11.68608 & 0.39 & 5.4 & 0.61 & 4.6 & 0.18 & 7.5 & 7.12\\
J1258-1800 & 0 & 0 & 194.65804 & -18.00317 & 0.80 & 8.2 & 0.77 & 7.6 & 0.48 & 13.2 & 9.84\\
J1303-5540 & 0 & 2 & 195.95435 & -55.67618 & 1.27 & 4.6 & 1.38 & 6.7 & 0.86 & 11.3 & 3.01\\
J1303-5540 & 1 & 2 & 195.95617 & -55.67482 & 0.64 & 3.4 & 0.88 & 1.7 & 0.39 & 5.1 & 3.18\\
J1305-1033 & 0 & 1 & 196.38803 & -10.55234 & 1.06 & 9.3 & 1.07 & 9.5 & 0.62 & 12.7 & 11.12\\
J1305-2850 & 0 & 1 & 196.28193 & -28.84626 & 0.59 & 4.5 & 0.56 & 4.3 & 0.34 & 8.5 & 11.50\\
J1307-5019 & 0 & 2 & 196.84773 & -50.32167 & 0.51 & 10.9 & 0.54 & 8.8 & 0.35 & 13.1 & 3.03\\
J1312-0424 & 0 & 1 & 198.20831 & -4.41343 & 1.06 & 5.7 & 1.01 & 5.2 & 0.38 & 8.9 & 13.65\\
J1312-7724 & 0 & 0 & 198.16392 & -77.40326 & 0.74 & 4.4 & 0.76 & 5.0 & 0.61 & 7.5 & 2.48\\
J1315-5334 & 0 & 1 & 198.76448 & -53.57458 & 1.92 & 9.6 & 1.95 & 8.9 & 1.08 & 15.9 & 9.73\\
J1321-2636 & 0 & 0 & 200.30724 & -26.60455 & 0.37 & 4.4 & 0.37 & 4.8 & 0.26 & 7.1 & 7.15\\
J1326-5256 & 0 & 2 & 201.70547 & -52.94098 & 0.48 & 6.0 & 0.51 & 5.1 & 0.38 & 10.2 & 3.96\\
J1331+3030 & 0 & 2 & 202.78390 & 30.50891 & 1.14 & 27.3 & 1.32 & 25.1 & 0.78 & 31.2 & 2.17\\
J1331+3030 & 1 & 1 & 202.78329 & 30.51195 & 0.68 & 5.8 & 0.71 & 7.5 & 0.33 & 13.2 & 10.77\\
J1332+0200 & 0 & 2 & 203.21977 & 2.01294 & 0.22 & 2.5 & 0.22 & 3.6 & 0.17 & 7.0 & 7.94\\
J1336-0829 & 0 & 0 & 204.03707 & -8.49706 & 0.34 & 5.3 & 0.33 & 4.0 & 0.21 & 6.6 & 9.74\\
J1336-0829 & 1 & 0 & 204.03515 & -8.49288 & 1.20 & 7.4 & 1.27 & 5.3 & 0.23 & 7.3 & 17.63\\
J1342-2900 & 0 & 1 & 205.56408 & -29.01347 & 0.23 & 3.2 & 0.21 & 3.0 & 0.17 & 5.3 & 6.68\\
J1354-1041 & 0 & 0 & 208.69445 & -10.68411 & 0.35 & 6.1 & 0.36 & 5.2 & 0.23 & 9.3 & 2.20\\
J1408-0752 & 0 & 0 & 212.23263 & -7.87777 & 1.46 & 7.3 & 1.46 & 6.7 & 0.36 & 12.4 & 16.43\\
J1408-2900 & 0 & 2 & 212.21244 & -29.00679 & 1.68 & 3.1 & 2.20 & 4.3 & 0.20 & 7.8 & 18.01\\
J1408-2900 & 1 & 2 & 212.20523 & -29.00598 & 1.47 & 27.2 & 1.81 & 27.3 & 0.92 & 36.3 & 5.15\\
J1420-0642 & 0 & 1 & 215.07378 & -6.70316 & 0.41 & 4.5 & 0.40 & 4.6 & 0.31 & 6.0 & 4.98\\
J1424-7241 & 0 & 0 & 216.21285 & -72.68751 & 0.76 & 4.8 & 0.75 & 4.1 & 0.47 & 5.9 & 5.55\\
J1448-1620 & 0 & 2 & 222.06219 & -16.33978 & 1.66 & 12.3 & 1.72 & 10.7 & 1.26 & 16.2 & 2.28\\
J1454-3747 & 0 & 1 & 223.61394 & -37.79076 & 2.29 & 17.8 & 2.37 & 23.7 & 1.56 & 36.3 & 6.44\\
J1532+2344 & 0 & 1 & 233.18916 & 23.73566 & 0.51 & 2.7 & 0.56 & 2.8 & 0.21 & 5.1 & 13.36\\
J1534-3526 & 0 & 1 & 233.73376 & -35.44260 & 2.26 & 8.4 & 2.34 & 8.3 & 0.25 & 12.4 & 19.89\\
J1550+0527 & 0 & 1 & 237.64214 & 5.45486 & 0.74 & 4.7 & 0.72 & 3.5 & 0.10 & 7.1 & 18.65\\
J1557-0001 & 0 & 1 & 239.46629 & -0.03153 & 0.39 & 7.9 & 0.39 & 6.3 & 0.24 & 12.4 & 7.78\\
J1604-4441 & 0 & 1 & 241.13297 & -44.69109 & 0.85 & 7.8 & 0.89 & 4.6 & 0.40 & 9.3 & 10.35\\
J1610-3958 & 0 & 1 & 242.59540 & -39.98440 & 0.52 & 7.6 & 0.54 & 6.4 & 0.16 & 11.5 & 12.90\\
J1619+2247 & 0 & 1 & 244.81538 & 22.79341 & 1.25 & 3.7 & 1.09 & 2.8 & 0.23 & 6.9 & 16.66\\
J1625-2527 & 0 & 1 & 246.44292 & -25.46531 & 1.00 & 1.6 & 0.95 & 7.4 & 0.16 & 14.2 & 18.61\\
J1626-2951 & 0 & 2 & 246.52418 & -29.85959 & 0.72 & 7.7 & 0.77 & 6.1 & 0.40 & 11.1 & 8.11\\
J1650-5044 & 0 & 1 & 252.56995 & -50.74877 & 0.28 & 5.1 & 0.32 & 4.6 & 0.17 & 7.9 & 7.52\\
J1708+0035 & 0 & 0 & 257.18377 & 0.58458 & 1.05 & 5.8 & 1.06 & 4.9 & 0.50 & 9.4 & 9.57\\
J1713-3418 & 0 & 1 & 258.28786 & -34.30689 & 1.08 & 7.0 & 1.17 & 5.6 & 0.36 & 7.9 & 11.56\\
J1720-3552 & 0 & 0 & 260.09025 & -35.88261 & 0.89 & 4.3 & 0.88 & 4.3 & 0.47 & 7.6 & 9.46\\
J1730+0024 & 0 & 1 & 262.64502 & 0.41199 & 0.36 & 3.8 & 0.37 & 4.7 & 0.30 & 7.8 & 5.34\\
J1733-1304 & 0 & 2 & 263.25813 & -13.08024 & 2.00 & 22.5 & 2.32 & 18.9 & 0.49 & 24.7 & 11.08\\
J1743-0350 & 0 & 0 & 265.99543 & -3.82977 & 1.70 & 3.5 & 1.97 & 2.8 & 0.26 & 5.2 & 17.46\\
J1744-3116 & 0 & 1 & 266.09454 & -31.27759 & 0.31 & 7.6 & 0.33 & 6.9 & 0.10 & 12.4 & 11.82\\
J1848+3219 & 0 & 0 & 282.08642 & 32.31649 & 1.62 & 5.5 & 1.55 & 5.5 & 0.41 & 9.7 & 17.38\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B6_catalogue_page4.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 6 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J1905+0952 & 0 & 1 & 286.41372 & 9.86622 & 0.31 & 5.0 & 0.27 & 4.1 & 0.11 & 7.3 & 13.43\\
J1905+0952 & 1 & 1 & 286.41713 & 9.87291 & 0.40 & 4.6 & 0.45 & 3.9 & 0.08 & 5.5 & 14.43\\
J1933-6942 & 0 & 1 & 293.37277 & -69.71623 & 1.69 & 8.4 & 1.69 & 8.3 & 0.95 & 11.2 & 8.83\\
J1945-0153 & 0 & 0 & 296.34445 & -1.88693 & 0.55 & 6.3 & 0.54 & 6.6 & 0.46 & 13.8 & 9.18\\
J2004-6347 & 0 & 1 & 301.11794 & -63.78801 & 0.82 & 5.5 & 1.05 & 4.4 & 0.35 & 6.0 & 10.11\\
J2025+3343 & 0 & 1 & 306.29620 & 33.71378 & 0.21 & 2.5 & 0.22 & 2.6 & 0.15 & 5.9 & 11.05\\
J2025-0735 & 0 & 2 & 306.41914 & -7.59742 & 3.86 & 68.4 & 3.88 & 76.7 & 2.90 & 118.4 & 2.21\\
J2040-5735 & 0 & 1 & 310.00896 & -57.59009 & 0.67 & 1.8 & 0.67 & 2.6 & 0.22 & 5.0 & 16.92\\
J2040-5735 & 1 & 1 & 310.00916 & -57.58442 & 0.87 & 7.8 & 0.96 & 6.9 & 0.45 & 10.2 & 10.51\\
J2051+1743 & 0 & 0 & 312.90060 & 17.72238 & 2.02 & 3.9 & 2.20 & 3.0 & 0.24 & 6.3 & 18.19\\
J2056-4714 & 0 & 2 & 314.06714 & -47.24762 & 0.22 & 2.1 & 0.26 & 5.2 & 0.11 & 11.4 & 4.58\\
J2056-5820 & 0 & 2 & 314.12431 & -58.34055 & 2.79 & 10.8 & 2.79 & 9.1 & 0.48 & 15.0 & 19.30\\
J2057-3734 & 0 & 0 & 314.42185 & -37.56989 & 0.34 & 2.2 & 0.36 & 3.3 & 0.38 & 7.1 & 9.63\\
J2101+0341 & 0 & 1 & 315.41029 & 3.69130 & 0.67 & 8.9 & 0.68 & 7.0 & 0.51 & 15.5 & 6.07\\
J2101+0341 & 1 & 1 & 315.41274 & 3.69246 & 0.37 & 6.2 & 0.42 & 4.2 & 0.20 & 6.2 & 3.67\\
J2105-4848 & 0 & 2 & 316.25961 & -48.81379 & 2.17 & 8.5 & 3.02 & 7.8 & 0.78 & 11.8 & 11.77\\
J2109-4110 & 0 & 1 & 317.38565 & -41.17213 & 0.49 & 6.7 & 0.52 & 6.4 & 0.27 & 9.9 & 7.20\\
J2114+2832 & 0 & 1 & 318.74406 & 28.54942 & 0.96 & 8.3 & 1.11 & 8.2 & 0.48 & 10.3 & 3.24\\
J2147+0929 & 0 & 2 & 326.79238 & 9.49708 & 0.29 & 6.0 & 0.32 & 4.0 & 0.13 & 5.2 & 2.82\\
J2147+0929 & 1 & 1 & 326.79318 & 9.49837 & 0.18 & 2.1 & 0.18 & 2.4 & 0.13 & 5.2 & 8.05\\
J2148+0657 & 0 & 1 & 327.02502 & 6.96006 & 0.55 & 19.6 & 0.57 & 15.5 & 0.34 & 40.1 & 8.44\\
J2151-3027 & 0 & 2 & 327.98176 & -30.46572 & 0.43 & 5.7 & 0.43 & 6.8 & 0.36 & 11.5 & 3.16\\
J2156-0037 & 0 & 1 & 329.06542 & -0.61442 & 2.03 & 10.6 & 2.02 & 9.3 & 0.30 & 16.5 & 18.98\\
J2156-0037 & 1 & 1 & 329.06132 & -0.61413 & 0.35 & 4.9 & 0.41 & 3.6 & 0.09 & 5.1 & 13.74\\
J2207-5346 & 0 & 2 & 331.93130 & -53.77735 & 1.01 & 11.9 & 1.10 & 8.1 & 0.55 & 15.6 & 5.02\\
J2212+0646 & 0 & 1 & 333.21086 & 6.77242 & 1.02 & 3.3 & 1.02 & 3.4 & 0.39 & 5.6 & 12.47\\
J2223-3137 & 0 & 1 & 335.84052 & -31.61882 & 0.28 & 6.1 & 0.29 & 6.0 & 0.26 & 10.7 & 5.79\\
J2226+0052 & 0 & 1 & 336.69545 & 0.86859 & 0.10 & 3.1 & 0.11 & 3.7 & 0.07 & 8.6 & 7.10\\
J2226+0052 & 1 & 1 & 336.69265 & 0.87133 & 0.31 & 6.3 & 0.32 & 17.4 & 0.20 & 25.0 & 7.08\\
J2226+0052 & 2 & 1 & 336.69643 & 0.87312 & 1.32 & 27.3 & 1.32 & 25.8 & 0.40 & 49.6 & 14.97\\
J2226+0052 & 3 & 1 & 336.69473 & 0.87419 & 0.34 & 2.4 & 0.35 & 6.4 & 0.08 & 9.5 & 16.03\\
J2229-0832 & 0 & 1 & 337.41717 & -8.54772 & 1.47 & 11.0 & 1.52 & 8.2 & 0.97 & 13.1 & 2.70\\
J2230-4416 & 0 & 1 & 337.73674 & -44.27617 & 0.23 & 4.8 & 0.26 & 2.6 & 0.14 & 6.0 & 5.92\\
J2247-3657 & 0 & 0 & 341.76484 & -36.95848 & 0.76 & 3.6 & 0.74 & 3.4 & 0.27 & 6.3 & 16.32\\
J2258-2758 & 0 & 1 & 344.52663 & -27.97609 & 0.47 & 7.3 & 0.49 & 7.3 & 0.14 & 13.2 & 13.90\\
J2258-2758 & 1 & 1 & 344.52213 & -27.97567 & 0.64 & 8.3 & 0.69 & 8.0 & 0.18 & 17.3 & 14.13\\
J2258-2758 & 2 & 2 & 344.52262 & -27.97193 & 0.31 & 9.1 & 0.33 & 2.5 & 0.15 & 13.6 & 7.45\\
J2301-0158 & 0 & 2 & 345.28242 & -1.96774 & 0.80 & 7.4 & 0.83 & 6.8 & 0.57 & 11.4 & 3.04\\
J2309-3059 & 0 & 2 & 347.31022 & -30.98737 & 0.76 & 6.5 & 0.83 & 4.8 & 0.42 & 7.8 & 2.49\\
J2323-0317 & 0 & 1 & 350.88568 & -3.28451 & 0.23 & 3.6 & 0.21 & 3.1 & 0.17 & 7.8 & 9.15\\
J2323-0617 & 0 & 0 & 350.90986 & -6.29672 & 2.55 & 5.9 & 3.00 & 4.7 & 0.37 & 7.7 & 15.71\\
J2335-0131 & 0 & 2 & 353.83605 & -1.51989 & 0.64 & 20.0 & 0.67 & 20.2 & 0.48 & 30.5 & 4.12\\
J2336-5236 & 0 & 1 & 354.04695 & -52.60554 & 0.57 & 5.6 & 0.59 & 4.2 & 0.36 & 8.3 & 8.23\\
J2353-3037 & 0 & 0 & 358.45184 & -30.62994 & 0.39 & 5.6 & 0.43 & 5.2 & 0.10 & 7.2 & 12.69\\
J2353-3037 & 1 & 0 & 358.44777 & -30.62711 & 0.53 & 10.5 & 0.57 & 7.9 & 0.16 & 11.2 & 10.90\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B6_catalogue_page5.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 6 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J2357-5311 & 0 & 1 & 359.46860 & -53.19167 & 0.59 & 6.3 & 0.59 & 6.8 & 0.11 & 15.9 & 17.84\\
J2359-3133 & 0 & 1 & 359.89817 & -31.56111 & 0.36 & 11.0 & 0.37 & 9.9 & 0.27 & 15.2 & 3.90\\
J1733-3722 & 0 & 1 & 263.31339 & -37.37359 & 2.19 & 35.9 & 2.24 & 38.2 & 1.39 & 61.3 & 7.48\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B7_catalogue_page0.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 7 }
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0019+2021 & 0 & 1 & 4.90603 & 20.36268 & 1.00 & 2.6 & 1.00 & 2.8 & 0.74 & 6.1 & 5.73\\
J0040-3243 & 0 & 1 & 10.07422 & -32.72509 & 0.62 & 5.1 & 0.60 & 4.7 & 0.48 & 6.5 & 4.26\\
J0103-6439 & 0 & 0 & 15.88705 & -64.65559 & 1.34 & 3.6 & 1.30 & 2.8 & 0.22 & 6.0 & 13.59\\
J0103-6439 & 1 & 1 & 15.89388 & -64.65369 & 0.35 & 3.0 & 0.34 & 3.2 & 0.19 & 5.3 & 7.57\\
J0106-2718 & 0 & 1 & 16.61070 & -27.30217 & 2.34 & 17.4 & 2.34 & 15.7 & 1.38 & 22.6 & 7.62\\
J0108+0135 & 0 & 2 & 17.16146 & 1.58221 & 0.91 & 11.9 & 0.93 & 9.2 & 0.58 & 16.8 & 4.40\\
J0108+0135 & 1 & 1 & 17.16065 & 1.58452 & 2.14 & 21.7 & 2.15 & 18.1 & 1.38 & 39.7 & 5.11\\
J0116-1136 & 0 & 1 & 19.05241 & -11.60520 & 0.48 & 2.2 & 0.49 & 3.2 & 0.40 & 5.6 & 3.40\\
J0120-2701 & 0 & 1 & 20.13225 & -27.02221 & 2.29 & 12.6 & 2.45 & 9.5 & 1.17 & 15.4 & 4.82\\
J0143-3200 & 0 & 0 & 25.79371 & -32.01861 & 1.75 & 4.1 & 1.79 & 3.3 & 0.28 & 5.0 & 11.29\\
J0215-0222 & 0 & 1 & 33.92460 & -2.38452 & 0.40 & 4.8 & 0.43 & 3.9 & 0.19 & 5.7 & 7.72\\
J0215-0222 & 1 & 2 & 33.92505 & -2.38318 & 0.23 & 3.7 & 0.25 & 3.4 & 0.17 & 5.1 & 2.71\\
J0217+0144 & 0 & 1 & 34.45504 & 1.74571 & 0.29 & 3.5 & 0.29 & 5.3 & 0.20 & 9.4 & 6.41\\
J0217+0144 & 1 & 1 & 34.45534 & 1.74885 & 0.28 & 3.2 & 0.26 & 3.1 & 0.14 & 6.9 & 7.85\\
J0217-0820 & 0 & 1 & 34.26137 & -8.35057 & 4.00 & 20.9 & 4.07 & 39.7 & 1.48 & 112.6 & 9.74\\
J0217-0820 & 1 & 1 & 34.26031 & -8.34988 & 0.47 & 7.1 & 0.55 & 1.5 & 0.16 & 12.6 & 7.72\\
J0217-0820 & 2 & 1 & 34.26220 & -8.34891 & 0.42 & 2.0 & 0.43 & 7.1 & 0.26 & 19.5 & 5.43\\
J0217-0820 & 3 & 1 & 34.26291 & -8.34891 & 3.93 & 22.6 & 4.13 & 60.2 & 1.65 & 125.9 & 7.47\\
J0217-0820 & 4 & 2 & 34.26137 & -8.34701 & 0.43 & 4.0 & 0.45 & 11.6 & 0.29 & 21.7 & 3.26\\
J0217-0820 & 5 & 1 & 34.25878 & -8.34577 & 0.36 & 2.2 & 0.36 & 3.4 & 0.09 & 7.1 & 11.19\\
J0217-0820 & 6 & 1 & 34.26227 & -8.34417 & 3.05 & 12.0 & 3.18 & 9.7 & 0.42 & 31.7 & 13.99\\
J0238+1636 & 0 & 1 & 39.66467 & 16.61517 & 0.32 & 2.1 & 0.30 & 1.8 & 0.10 & 5.2 & 9.67\\
J0238+1636 & 1 & 1 & 39.66496 & 16.61565 & 0.84 & 6.1 & 0.86 & 6.3 & 0.22 & 12.1 & 9.93\\
J0239+0416 & 0 & 0 & 39.96117 & 4.27438 & 1.91 & 2.4 & 1.93 & 1.9 & 0.57 & 5.1 & 10.82\\
J0239-0234 & 0 & 1 & 39.93740 & -2.57801 & 0.49 & 6.0 & 0.85 & 4.6 & 0.17 & 5.4 & 7.45\\
J0241-0815 & 0 & 0 & 40.27090 & -8.25407 & 0.08 & 0.6 & 0.08 & 0.7 & 0.10 & 5.6 & 6.91\\
J0241-0815 & 1 & 1 & 40.27006 & -8.25416 & 1.48 & 27.5 & 1.48 & 22.5 & 0.87 & 50.8 & 5.79\\
J0245-4459 & 0 & 0 & 41.47734 & -44.99654 & 1.88 & 2.9 & 1.89 & 3.1 & 0.92 & 6.2 & 9.28\\
J0253-5441 & 0 & 1 & 43.37232 & -54.69621 & 1.50 & 18.9 & 1.55 & 14.3 & 1.01 & 24.2 & 5.31\\
J0259+0747 & 0 & 1 & 44.86363 & 7.79675 & 1.55 & 5.4 & 1.52 & 4.7 & 0.48 & 8.9 & 9.12\\
J0348-1610 & 0 & 1 & 57.16558 & -16.17329 & 1.28 & 4.4 & 1.26 & 3.3 & 0.43 & 5.4 & 9.08\\
J0348-2749 & 0 & 2 & 57.15950 & -27.82072 & 1.13 & 24.1 & 1.14 & 17.1 & 0.81 & 52.1 & 2.05\\
J0348-2749 & 1 & 1 & 57.15578 & -27.82012 & 3.48 & 11.4 & 4.33 & 5.1 & 0.20 & 12.8 & 10.12\\
J0403-2444 & 0 & 1 & 60.92389 & -24.73775 & 0.49 & 4.7 & 0.55 & 3.5 & 0.19 & 5.1 & 7.42\\
J0406-3826 & 0 & 0 & 61.74450 & -38.44142 & 0.99 & 3.8 & 0.96 & 3.3 & 0.67 & 6.0 & 4.32\\
J0406-3826 & 1 & 0 & 61.74334 & -38.44100 & 2.45 & 6.3 & 2.73 & 4.9 & 0.78 & 7.0 & 7.46\\
J0418+3801 & 0 & 1 & 64.59237 & 38.02625 & 4.42 & 4.1 & 4.62 & 3.6 & 1.31 & 5.5 & 10.60\\
J0423-0120 & 0 & 1 & 65.81295 & -1.34118 & 6.06 & 4.8 & 5.29 & 2.5 & 0.22 & 11.4 & 11.47\\
J0426+2327 & 0 & 1 & 66.73114 & 23.46268 & 0.51 & 3.2 & 0.56 & 2.9 & 0.20 & 5.0 & 7.00\\
J0438+3004 & 0 & 2 & 69.51982 & 30.07903 & 0.97 & 14.5 & 1.21 & 14.1 & 0.43 & 19.8 & 2.71\\
J0440-4333 & 0 & 1 & 70.06812 & -43.55140 & 5.02 & 9.4 & 5.26 & 7.7 & 1.18 & 11.2 & 9.72\\
J0440-4333 & 1 & 1 & 70.07275 & -43.55022 & 3.37 & 7.3 & 3.44 & 6.6 & 1.47 & 13.9 & 8.38\\
J0453-2807 & 0 & 1 & 73.31066 & -28.12590 & 1.09 & 11.3 & 1.11 & 12.8 & 0.70 & 17.1 & 4.25\\
J0457-2324 & 0 & 1 & 74.26509 & -23.41671 & 1.47 & 4.8 & 1.39 & 3.0 & 0.45 & 6.2 & 10.15\\
J0506-6109 & 0 & 0 & 76.68001 & -61.16139 & 0.68 & 2.6 & 0.65 & 3.0 & 0.71 & 6.2 & 5.69\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B7_catalogue_page1.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 7 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J0526-4830 & 0 & 1 & 81.57237 & -48.51208 & 1.00 & 11.6 & 1.13 & 9.8 & 0.33 & 12.0 & 9.62\\
J0529-7245 & 0 & 1 & 82.37026 & -72.75626 & 0.48 & 4.8 & 0.53 & 5.0 & 0.19 & 7.5 & 7.96\\
J0538-4405 & 0 & 1 & 84.71275 & -44.08509 & 0.53 & 6.4 & 0.60 & 5.1 & 0.17 & 10.2 & 7.97\\
J0539+1433 & 0 & 1 & 84.92556 & 14.56232 & 2.57 & 25.7 & 2.62 & 28.6 & 1.99 & 37.5 & 3.59\\
J0542-0913 & 0 & 1 & 85.72926 & -9.22415 & 5.15 & 3.9 & 5.35 & 3.7 & 0.92 & 6.0 & 13.30\\
J0550-5732 & 0 & 1 & 87.53634 & -57.53793 & 1.29 & 14.1 & 1.29 & 13.1 & 0.45 & 23.0 & 10.47\\
J0635-7516 & 0 & 2 & 98.95542 & -75.27123 & 0.61 & 2.5 & 0.73 & 2.5 & 0.12 & 5.2 & 10.66\\
J0643+0857 & 0 & 1 & 100.85845 & 8.95896 & 0.45 & 4.9 & 0.49 & 4.2 & 0.17 & 5.5 & 8.44\\
J0643+0857 & 1 & 1 & 100.85839 & 8.95985 & 0.49 & 6.6 & 0.49 & 5.8 & 0.27 & 9.0 & 6.89\\
J0654-1053 & 0 & 0 & 103.54271 & -10.89482 & 1.84 & 4.4 & 1.78 & 2.8 & 0.50 & 5.4 & 7.21\\
J0831+0429 & 0 & 1 & 127.95458 & 4.49515 & 6.17 & 22.6 & 6.16 & 22.4 & 3.45 & 40.3 & 4.80\\
J0853+0654 & 0 & 1 & 133.45024 & 6.91040 & 0.74 & 2.7 & 0.77 & 2.2 & 0.21 & 5.3 & 9.98\\
J0853+0654 & 1 & 1 & 133.45061 & 6.91176 & 2.62 & 25.9 & 2.65 & 26.2 & 2.05 & 50.2 & 4.93\\
J0854+2006 & 0 & 1 & 133.70592 & 20.10952 & 5.34 & 6.3 & 5.16 & 4.8 & 0.52 & 14.7 & 8.50\\
J0904-5735 & 0 & 2 & 136.22241 & -57.58428 & 14.86 & 19.9 & 16.84 & 19.2 & 4.85 & 22.5 & 2.85\\
J0922-3959 & 0 & 2 & 140.69345 & -39.99367 & 1.67 & 5.5 & 1.77 & 3.7 & 0.84 & 8.8 & 2.13\\
J0948+0022 & 0 & 1 & 147.24085 & 0.37496 & 0.21 & 3.4 & 0.21 & 8.0 & 0.10 & 13.7 & 8.44\\
J0948+0022 & 1 & 1 & 147.23894 & 0.37660 & 0.23 & 5.1 & 0.29 & 4.3 & 0.06 & 8.9 & 10.20\\
J1008+0621 & 0 & 1 & 152.00257 & 6.35506 & 0.18 & 6.1 & 0.21 & 4.4 & 0.10 & 5.2 & 4.20\\
J1010-0200 & 0 & 2 & 152.71662 & -2.00567 & 0.13 & 3.3 & 0.15 & 3.5 & 0.07 & 5.2 & 4.89\\
J1010-0200 & 1 & 1 & 152.71259 & -2.00522 & 0.62 & 13.8 & 0.61 & 6.3 & 0.22 & 16.7 & 9.71\\
J1010-0200 & 2 & 1 & 152.71301 & -2.00267 & 0.75 & 4.9 & 0.76 & 6.4 & 0.12 & 9.4 & 12.92\\
J1047-6217 & 0 & 1 & 161.92949 & -62.28652 & 0.34 & 2.1 & 0.40 & 2.6 & 0.45 & 6.3 & 3.27\\
J1048-1909 & 0 & 1 & 162.02851 & -19.15816 & 0.62 & 4.9 & 0.75 & 3.2 & 0.19 & 5.5 & 7.08\\
J1048-1909 & 1 & 1 & 162.02722 & -19.15722 & 0.68 & 2.9 & 0.64 & 2.2 & 0.22 & 6.5 & 9.82\\
J1058+0133 & 0 & 1 & 164.62389 & 1.56590 & 4.39 & 24.2 & 4.40 & 10.2 & 3.26 & 130.0 & 2.46\\
J1107-4449 & 0 & 1 & 166.78457 & -44.81682 & 0.42 & 3.5 & 0.43 & 5.7 & 0.24 & 10.5 & 8.26\\
J1118+1234 & 0 & 2 & 169.73830 & 12.57869 & 1.36 & 7.9 & 1.44 & 8.1 & 0.89 & 13.9 & 2.23\\
J1118+1234 & 1 & 1 & 169.74092 & 12.57935 & 2.88 & 10.0 & 2.99 & 10.3 & 1.14 & 17.9 & 8.59\\
J1147-0724 & 0 & 1 & 176.96368 & -7.41031 & 1.75 & 10.5 & 1.83 & 8.6 & 0.91 & 15.8 & 5.69\\
J1148+1840 & 0 & 1 & 177.15968 & 18.67131 & 3.04 & 19.6 & 2.93 & 19.0 & 0.71 & 31.5 & 10.97\\
J1150+2417 & 0 & 1 & 177.57908 & 24.29911 & 0.98 & 8.3 & 0.98 & 8.4 & 0.79 & 12.7 & 4.34\\
J1159+2914 & 0 & 1 & 179.88616 & 29.24631 & 3.58 & 4.0 & 3.49 & 3.8 & 0.90 & 6.1 & 11.41\\
J1209-2406 & 0 & 1 & 182.25931 & -24.10733 & 1.31 & 6.4 & 1.30 & 5.8 & 0.76 & 8.8 & 6.32\\
J1215+1654 & 0 & 0 & 183.76422 & 16.91087 & 0.95 & 5.8 & 1.03 & 4.1 & 0.31 & 5.2 & 8.23\\
J1224+0330 & 0 & 0 & 186.21831 & 3.51327 & 6.62 & 62.6 & 6.67 & 51.8 & 4.83 & 109.4 & 2.54\\
J1243+1622 & 0 & 2 & 190.99026 & 16.37978 & 1.69 & 9.5 & 1.77 & 5.9 & 1.01 & 19.1 & 6.18\\
J1243+1622 & 1 & 2 & 190.98911 & 16.38387 & 8.44 & 41.9 & 8.70 & 28.7 & 2.89 & 54.8 & 9.35\\
J1245-1616 & 0 & 1 & 191.47387 & -16.27741 & 0.43 & 5.1 & 0.46 & 3.6 & 0.21 & 5.3 & 7.05\\
J1303-5540 & 0 & 2 & 195.95436 & -55.67619 & 0.72 & 4.9 & 0.76 & 4.6 & 0.57 & 8.5 & 3.05\\
J1305-1033 & 0 & 1 & 196.38804 & -10.55232 & 4.54 & 11.1 & 4.59 & 9.3 & 1.09 & 16.1 & 11.21\\
J1331+3030 & 0 & 2 & 202.78382 & 30.50886 & 0.67 & 7.6 & 0.71 & 5.6 & 0.38 & 6.8 & 2.44\\
J1331+3030 & 1 & 1 & 202.78326 & 30.51193 & 1.58 & 5.8 & 1.64 & 4.9 & 0.44 & 8.0 & 10.73\\
J1424-6807 & 0 & 1 & 216.23004 & -68.13232 & 1.60 & 13.1 & 1.62 & 11.3 & 1.33 & 24.4 & 2.64\\
J1438-3122 & 0 & 0 & 219.54464 & -31.37325 & 2.52 & 14.0 & 2.59 & 12.1 & 1.50 & 21.4 & 4.91\\

\hline
\end{tabular}
\end{table}
\end{landscape}


==> data/B7_catalogue_page2.tex <==

\begin{landscape}
\begin{table}
\caption{The detections in ALMA band 7 continued}
\begin{tabular}{cccccccccccc}
\hline
Field & index & type & R.A. & Dec. & Aperture flux & Aperture SNR & Gaussian flux & Gaussian SNR & Peak flux & Peak SNR & Radial distance\\
      & & & deg & deg & mJy & & mJy & & mJy & mJy\,beam$^{-1}$ & arcsec \\
\hline
J1512+0203 & 0 & 2 & 228.06606 & 2.05286 & 4.19 & 26.1 & 4.93 & 26.4 & 1.73 & 25.9 & 6.89\\
J1512+0203 & 1 & 2 & 228.06580 & 2.05412 & 0.67 & 2.3 & 0.70 & 4.7 & 0.54 & 8.1 & 2.28\\
J1512+0203 & 2 & 1 & 228.06258 & 2.05574 & 1.21 & 1.6 & 1.40 & 3.5 & 0.36 & 5.4 & 11.45\\
J1549+0237 & 0 & 0 & 237.37070 & 2.61421 & 5.36 & 4.5 & 7.86 & 3.5 & 0.69 & 5.0 & 12.23\\
J1604-4441 & 0 & 1 & 241.13303 & -44.69111 & 1.48 & 8.1 & 1.53 & 6.8 & 0.05 & 7.3 & 10.41\\
J1610-3958 & 0 & 1 & 242.59538 & -39.98438 & 1.53 & 7.7 & 1.67 & 6.7 & 0.28 & 16.1 & 12.83\\
J1610-3958 & 1 & 1 & 242.58732 & -39.98409 & 0.63 & 4.0 & 0.74 & 6.6 & 0.13 & 7.3 & 11.49\\
J1625-2527 & 0 & 1 & 246.44612 & -25.45883 & 0.28 & 1.4 & 0.30 & 1.9 & 0.12 & 6.0 & 6.96\\
J1626-2951 & 0 & 2 & 246.52417 & -29.85962 & 0.37 & 3.2 & 0.36 & 2.6 & 0.19 & 6.5 & 8.20\\
J1650-5044 & 0 & 1 & 252.57108 & -50.74868 & 0.36 & 2.6 & 0.37 & 2.8 & 0.23 & 5.2 & 8.14\\
J1650-5044 & 1 & 1 & 252.56996 & -50.74874 & 0.96 & 8.6 & 1.08 & 6.5 & 0.35 & 8.1 & 7.42\\
J1709-3525 & 0 & 2 & 257.32856 & -35.42248 & 5.45 & 9.9 & 6.58 & 9.3 & 2.19 & 9.0 & 2.59\\
J1716+2152 & 0 & 0 & 259.04574 & 21.86908 & 1.63 & 5.4 & 1.66 & 5.7 & 1.20 & 8.3 & 5.81\\
J1730+0024 & 0 & 1 & 262.64504 & 0.41198 & 1.13 & 2.9 & 1.01 & 2.8 & 0.80 & 6.1 & 5.28\\
J1733-1304 & 0 & 1 & 263.26070 & -13.08370 & 1.32 & 2.7 & 1.71 & 4.0 & 0.15 & 5.9 & 11.96\\
J1733-1304 & 1 & 2 & 263.25808 & -13.08025 & 1.57 & 7.3 & 1.92 & 5.5 & 0.22 & 9.0 & 11.25\\
J1733-3722 & 0 & 1 & 263.31339 & -37.37357 & 12.92 & 37.1 & 13.56 & 41.0 & 3.18 & 61.3 & 7.51\\
J1742-1517 & 0 & 1 & 265.54738 & -15.28874 & 0.56 & 0.9 & 0.55 & 1.3 & 0.41 & 5.4 & 10.58\\
J1744-3116 & 0 & 1 & 266.09453 & -31.27758 & 1.16 & 8.0 & 1.24 & 7.3 & 0.22 & 12.3 & 11.83\\
J1832-2039 & 0 & 1 & 278.04611 & -20.66149 & 0.46 & 4.2 & 0.46 & 4.2 & 0.18 & 8.2 & 6.82\\
J1851+0035 & 0 & 1 & 282.94414 & 0.59405 & 0.19 & 1.3 & 0.21 & 1.9 & 0.14 & 5.3 & 6.50\\
J1851+0035 & 1 & 2 & 282.94401 & 0.59134 & 0.84 & 16.7 & 1.13 & 12.3 & 0.46 & 14.9 & 4.32\\
J1933-6942 & 0 & 1 & 293.37274 & -69.71626 & 4.17 & 6.9 & 4.15 & 6.6 & 1.83 & 10.4 & 8.86\\
J1938+0448 & 0 & 1 & 294.62820 & 4.80407 & 1.37 & 11.2 & 1.52 & 10.3 & 0.56 & 11.5 & 3.36\\
J2025-0735 & 0 & 2 & 306.41914 & -7.59742 & 3.12 & 23.7 & 3.15 & 21.1 & 2.59 & 34.5 & 2.21\\
J2040-5735 & 0 & 1 & 310.00920 & -57.58438 & 2.67 & 11.5 & 2.75 & 8.2 & 0.88 & 11.7 & 10.66\\
J2101+0341 & 0 & 1 & 315.41029 & 3.69129 & 1.79 & 11.2 & 1.82 & 11.7 & 1.39 & 25.8 & 6.11\\
J2109-4110 & 0 & 1 & 317.38565 & -41.17215 & 1.37 & 6.4 & 1.44 & 9.5 & 0.89 & 13.1 & 7.20\\
J2206-0031 & 0 & 1 & 331.67906 & -0.51967 & 0.68 & 4.3 & 0.67 & 4.7 & 0.35 & 10.1 & 9.53\\
J2206-0031 & 1 & 1 & 331.67862 & -0.51891 & 6.43 & 52.1 & 6.79 & 43.4 & 2.15 & 62.0 & 8.38\\
J2207-5346 & 0 & 2 & 331.93136 & -53.77735 & 0.64 & 2.9 & 0.55 & 3.8 & 0.42 & 5.9 & 5.00\\
J2226+0052 & 0 & 1 & 336.69541 & 0.86860 & 0.24 & 2.9 & 0.27 & 3.4 & 0.15 & 6.0 & 6.96\\
J2226+0052 & 1 & 1 & 336.69263 & 0.87132 & 0.81 & 10.6 & 0.86 & 10.4 & 0.41 & 16.0 & 7.11\\
J2229-0832 & 0 & 1 & 337.41715 & -8.54771 & 2.56 & 17.4 & 2.51 & 16.3 & 2.06 & 32.1 & 2.74\\
J2315-5018 & 0 & 0 & 348.93070 & -50.30847 & 3.66 & 4.1 & 3.62 & 3.8 & 0.81 & 7.7 & 13.03\\
J2323-0317 & 0 & 1 & 350.88481 & -3.28722 & 0.53 & 4.3 & 0.57 & 3.7 & 0.15 & 5.6 & 10.80\\
J2323-0317 & 1 & 1 & 350.88570 & -3.28452 & 0.59 & 7.1 & 0.58 & 8.0 & 0.30 & 11.1 & 9.23\\
J2348-1631 & 0 & 0 & 357.01224 & -16.51994 & 1.09 & 4.7 & 1.31 & 3.6 & 0.29 & 5.2 & 4.72\\
J2359-3133 & 0 & 1 & 359.89816 & -31.56113 & 0.48 & 3.7 & 0.44 & 3.8 & 0.38 & 8.9 & 3.84\\
J2148+0657 & 0 & 1 & 327.02502 & 6.96006 & 1.59 & 28.2 & 1.62 & 27.5 & 0.72 & 45.0 & 8.45\\

\hline
\end{tabular}
\end{table}
\end{landscape}

